To be or not to be intrusive? The solution of parametric and stochastic equations - the "plain vanilla" Galerkin case

In parametric equations - stochastic equations are a special case - one may want to approximate the solution such that it is easy to evaluate its dependence of the parameters. Interpolation in the parameters is an obvious possibility, in this context often labeled as a collocation method. In the frequent situation where one has a "solver" for the equation for a given parameter value - this may be a software component or a program - it is evident that this can independently solve for the parameter values to be interpolated. Such uncoupled methods which allow the use of the original solver are classed as "non-intrusive". By extension, all other methods which produce some kind of coupled system are often - in our view prematurely - classed as "intrusive". We show for simple Galerkin formulations of the parametric problem - which generally produce coupled systems - how one may compute the approximation in a non-intusive way.

==> common/pdfsetup.tex <==
% RCSID:       $Id: pdfsetup.tex 36 2007-04-12 15:00:01Z opajonk $
% Author:      Oliver Pajonk
% Contact:     o.pajonk@tu-bs.de, oliver@oliverpajonk.de

% Setup PDF-Latex to fill in all relevant metadata into a PDF file
%
% Needs: - you have to declare \theauthor, \thetitle, \thesubject
%           \pdflinkcolor and  \thekeywords before including this file

% The following package defines \ifpdf properly even with MikTeX 2.5
\usepackage{ifpdf}

\ifpdf
  \usepackage[pdftex,
       colorlinks=true,		% use links with color instead of boxes
       bookmarksnumbered,	% bookmarks have numbers in front of topic
       bookmarksopen,		% opens the bookmarks when the PDF is opened
       pdfstartview=FitH,	% opens the PDF with 'fit width' view
       linkcolor=\pdflinkcolor,	% standard red
       citecolor=\pdflinkcolor,	% standard green
       urlcolor=\pdflinkcolor,	% standard cyan
       filecolor=\pdflinkcolor,	% ?
       hyperindex,		% ?
       plainpages=false,	% ?
       breaklinks=true,		% allow links to break across lines!
       pdfpagelabels, %?
       hypertexnames=true,
%        linktocpage=true  % if enabled the link in toc is placed on the number rather than on the text
     ]{hyperref}
     \pdfinfo{
        /Title (\thetitle)
        /Author (\theauthor)
        /Subject (\thesubject)
        /Keywords (\thekeywords)}
     \usepackage[dvipdf]{graphicx}
	 \usepackage[pdftex]{thumbpdf}
\else
  \usepackage[
    colorlinks=true,
    linkcolor=\pdflinkcolor,
    hyperindex,
    plainpages=false
  ]{hyperref}
  \usepackage[dvips]{graphicx}
\fi

\hypersetup{a5paper,
            colorlinks,
            linkcolor=\pdflinkcolor,
            citecolor=\pdflinkcolor,
            urlcolor=\pdflinkcolor,
            pdftitle={\thetitle},
            pdfauthor={\theauthor},
            pdfsubject={\thesubject},
            pdfkeywords={\thekeywords},
            pdfproducer={\theauthor~using \LaTeXe}}

